Foraging-based Optimization of Menu Systems

Computational design of menu systems has been solved in limited cases such as the linear menu (list) as an assignment task, where commands are assigned to menu positions while optimizing for for users selection performance and distance of associated items. We show that this approach falls short with larger, hierarchically organized menu systems, where one must also take into account how users navigate hierarchical structures. This paper presents a novel integer programming formulation that models hierarchical menus as a combination of the exact set covering problem and the assignment problem. It organizes commands into ordered groups of ordered groups via a novel objective function based on information foraging theory. It minimizes, on the one hand, the time required to select a command whose location is known from previous usage and, on the other, the time wasted in irrelevant parts of the menu while searching for commands whose location is not known. The convergence of these two factors yields usable, well-ordered command hierarchies from a single model. In generated menus, the lead (first) elements of a group or tab are good indicators of the remaining contents, thereby facilitating the search process. In a controlled usability evaluation, the performance of computationally designed menus was 25 faster than existing commercial designs with respect to selection time. The algorithm is efficient for large, representative instances of the problem. We further show applications in personalization and adaptation of menu systems.

==> Conclusion.tex <==
Our motivation for revisiting menu design was their persisting popularity and prevalence as interfaces.  % I don't see this text in the rendered PDF file, so I haven't proofed this file. -als
The design of menus strongly affects the usability and learnability of the computing applications we use on a daily basis.
So far most if not all menu systems are designed manually.
However, even a cursory exploration of existing menus reveals that the present-day design practices have not reached a state where usable menus could be produced reliably.

This paper has shown significant progress with a reformulation of the optimization objective. 
The wide variety of factors involved in menu design (e.g., number of tabs, lengths of individual tabs, number of groups within a tab, lengths of individual groups, associativity within groups/tabs, frequency of usage of commands, etc.) has previously made it difficult to formulate a reliable objective and even identify a good solution from a poor one. 
The key insight has been to solve assignment and set covering problems simultaneously while taking into account how optimal foraging performance is affected by design.
Despite the new, more complex objective, the new formulation provides results within comparable time with the assignment-only approach. 

Computational solutions like the one explored here could improve the productivity and enjoyability of computer use, facilitate the work of designers, and drive design automation.
While human designers can excel in creative problem-solving, 
they would benefit from computational support especially in combinatorially challenging design problems.
Both novice and expert designers can generate only a few candidate designs per iteration.
Moreover, they easily get fixated on one solution.
Designing good menus is a skill that requires years of practice. 
In the future, the methods we propose in this paper could be integrated in design tools and application development environments to facilitate menu design. 
Moreover, 
menu designs could be adapted automatically, assuming that data is available on frequency of access (or interest) and associativity of commands.

% From Abstract:
%We argue that computational methods that can autonomously design user interfaces is an important step forward in human--machine interaction and in improving the usability of complex computing systems.


==> DesignConsiderations.tex <==
This section discusses the nuances of the menu organization that will make the
resulting menu structures better amenable to its users. At the outset, we argue
that two major factors govern the efficacy of teh layout in any candidate
solution:  % This file's content doesn't seem to be used in the rendered material, so I've not edited it. -als
\begin{itemize}
\item \textit{Selection performance}: How quickly can a user find a desired
item, assuming that the user already known the menu quite well?
\item \textit{Learnability}: How easily can an average user learn a
new/unfamiliar menu?
\end{itemize}

These two criteria are complementary to each other: Assuming that a user
is seeing a specific menu structure for the first time, usage of the menu
implies a search for the desired commands. This search depends on the context with other commands,
as well as the expertise of the user. Here, the user is guided by
semantic cues (names of tabs and then closely associated commands). After the user has used
the menu for some period of time, the user starts memorizing the
locations of frequently used commands. Thereafter, there is no process
for searching the commands; the user will directly navigated to the
required tab and cluster. The effort in doing so depends only on the
position of the command. The performance in such a \textit{direct access} case
is governed by the Fitt's law \citep{fitts1954information} that models the time
cost of selecting a command starting from a given location. 

The dual criteria (Fitt's law performance criterion and learnability criterion)
manifest themselves in a variety of different ways:
\begin{itemize}
  \item \textit{Frequency of usage}: The commands that are used more often
  should be placed such that the Fitt's law performance criterion is best
  satisfied for them. For the purposes of this discussion, we assume that the
  reference location for the user is the top-left corner (first tab) of the
  menubar. We also assume that the problem data instance specifies the relative
  frequency of usage $F_i$ for every command $i$. Then the high-frequency
  commands can be identified easily. It is expected that the \textbf{optimized
  layouts place the high frequency commands at the most accessible
  locations}.
  \item \textit{Association between a pair of commands}: We expect the problem
  data instance to specify the relative logical interconnection between every
  pair of commands. We denote this quantity as the association score $A_{ij}$
  between commands $i$ and $j$. Now, consider that the score $A_{ij}$ for some
  specific pair of commands $i$ and $j$ is relatively very high among all pairs.
  Further, let us assume that the user has recently used command $i$ and
  remembers its location in the menu. Now, the user seeks to use command $j$.
  Due to the semantic interconnection between $i$ and $j$, the user logically
  expects that $j$ should appear in close vicinity of $i$. This means that
  \textbf{Pairs of commands with higher association scores should be
  located in close vicinity of each other}.
  \item \textit{Association within clusters and groups}: Consider that there
  exists a cluster that contains commands $i$,$j$ and $k$. Further, the 
  association between the pair $i,j$ is quite low. Similarly, the association
  for pairs $i,k$ and between $k,j$ is also quite low. Then, it may be better
  to split up cluster $i,j,k$ and redistribute the commands at locations where
  they have a better association with other commands. The same logic can be
  extended to tabs also. In general, \textbf{clusters (or tabs) should be
  constituted by commands which have a strong association with each other}.
  \item \textit{Ordering of clusters and tabs}: Consider that the
  constituent commands of a cluster have been determined and the relative ordering is to be
  decided. Then, Fitt's law indicates that the highest frequency commands within
  this cluster be placed at relatively upper/higher locations within this
  cluster to be better accessible. The low-usage constituents (low-frequency
  commands) within this cluster are better placed lower down the order. In
  general, \textbf{tabs and clusters} should be ordered in descending order
  of relative frequency. 
  \item \textit{Poorly associated commands}: It is quite likely that certain
  commands in the menu are not logically interrelated to any other commands.
  These may indicate some specific or unique actions possible for the specific
  application. Irrespective of the lack of interrelation (lower association
  score), it is still neccessary to place these commands somewhere in the menu.
  Then, it may be a good strategy to collect all such \textit{weird}
  commands and make a special cluster to place them. Naturally, the
  internal association within this special cluster will be quite low. We allow
  this \textbf{one special weird cluster to accommodate several unrelated weird
  elements}. The size of the weird cluster needs to be balanced carefully: A
  very large weird cluster will make search of commands challenging. But we also
  do not want the presence of weird commands to contaminate and impair
  other well-associated clusters. 
  \item \textit{Preferential positioning}: We note that menus are beng used
  as GUI elements since several decades now. Over this period, it has become
  an established norm to place some often-used commands in some specific
  locations. For example, assistive commands like \textit{Help} and reflective
  commands like \textit{About \ldots} are customarily placed in the last
  (rightmost) tab. On the contrary file (or session) handling
  commands like \textit{Open, Save, Exit} are placed in the first (or leftmost)
  tab. While these customary positions do not bring any specific benefits
  from the perspective of Fitt's law or association, it is still incumbent upon
  the optimizer to \textbf{adhere to the preferential positioning norms of
  commonly used commands} as far as possible.
\end{itemize}

Each of the design considerations listed above will be translated to suitable
objective or constraint in the mathematical models discussed in this paper.


==> KeywordData.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121.10003124.10010865</concept_id>
<concept_desc>Human-centered computing~Graphical user interfaces</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003121.10003126</concept_id>
<concept_desc>Human-centered computing~HCI theory, concepts and models</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003123.10011758</concept_id>
<concept_desc>Human-centered computing~Interaction design theory, concepts and paradigms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003121.10003125.10010873</concept_id>
<concept_desc>Human-centered computing~Pointing devices</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003121.10003128.10011754</concept_id>
<concept_desc>Human-centered computing~Pointing</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010148.10010149.10003628</concept_id>
<concept_desc>Computing methodologies~Combinatorial algorithms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010405.10010481.10003558</concept_id>
<concept_desc>Applied computing~Consumer products</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Graphical user interfaces}
\ccsdesc[500]{Human-centered computing~HCI theory, concepts and models}
\ccsdesc[500]{Human-centered computing~Interaction design theory, concepts and paradigms}
\ccsdesc[300]{Human-centered computing~Pointing devices}
\ccsdesc[300]{Human-centered computing~Pointing}
\ccsdesc[500]{Computing methodologies~Combinatorial algorithms}
\ccsdesc[100]{Applied computing~Consumer products}
 
\keywords{
Combinatorial optimization,
Integer programming,
Computational design,
User interfaces,
Menu systems,
Information foraging,
Human-computer interaction
}


==> Results_New_Narrative.tex <==
This section assesses the quality of optimized designs and reports numerical performance.  % The content of this file doesn't seem to be in use, so the only edits are a few that I made to all files earlier on.  -als

\input{DataInstances}

\subsection{Numerical Performance}
The MILP formulations were coded using Java\texttrademark\ SE (build 1.8)
programming language. The solving for this formulation has been handled via the
IBM\texttrademark \ Cplex\texttrademark\ 12.6.2 solver. The computer hardware
utilized is 8-core 64-bit Intel\texttrademark\ i7\texttrademark\ processor at
2.8Ghz with 16 GB RAM. The MIP solver is used with Concert\texttrademark\
technology in conjunction with several customized callbacks. 

Computation times for the three cases are given in Table \ref{TablecomputationalTime}. These times are reported as averages of multiple computational executions with different
values of weight functions $\lambda$ and $\Phi$. We note that for extreme values of
$\lambda$ and $\Phi$, we will observe much shorter computational efforts. 

\begin{table}[!htbp]
  \centering
  \caption{Computation times for optimal solutions by the optimizer, separately for two different evaluative functions}
\begin{tabular}{l|c|c}
    \multicolumn{3}{c}{Average Time (minutes) required to find optimal
    solution}
    \\
    \hline
    \hline
    Application & Dual-Objective Approach & Information Foraging Approach \\
    \hline
    Windows Notepad & 17  & 22 \\
    Adode Acrobat Viewer & 960 & 1201 \\
    Firefox Browser & 1145 & 1633 \\
    \hline
    \end{tabular}%
  \label{TablecomputationalTime}%
\end{table}%

The computational times reported appear to be satisfactory for the purposes of
the current problem.
We assume that for professional software, software vendors should be ready to
invest a few hours or even a few weeks of computational effort to ensure that
they get the best possible menu design.
Secondly, the data show that using IFT does not significantly hamper performance
over the earlier dual-objective approach.

\subsection{Optimized Menu Designs}
We present optimized layouts generated using the algorithms and
formulations discussed earlier for the data instances designed in Subsection
\ref{Task instances}. The results for the three data instances using the
dual-objective approach MRF are provided in Figures \ref{NotepadClassical.PNG},
\ref{FirefoxClassical.PNG} and \ref{AcrobatClassical.PNG}.
The layouts resulting from the information foraging approach
are provided in figures \ref{NotepadResult.PNG}, \ref{FirefoxResult.PNG} and
\ref{AcrobatResult.PNG}. To facilitate comparison, we have provided
the unoptimized (existing) layouts also, in figures \ref{NotepadUnoptimized.PNG},
\ref{FirefoxUnoptimized.PNG} and \ref{AcrobatUnoptimized.PNG}.

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{NotepadUnoptimized.PNG}}
\caption{The unoptimized menu for the Windows Notepad\texttrademark\ text editor}
\label{NotepadUnoptimized.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{NotepadClassical.PNG}}
\caption{Dual-Objective MRF Approach: A menu optimized for the Windows Notepad\texttrademark\ text editor}
\label{NotepadClassical.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{NotepadResult.PNG}}
\caption{IFT-based Approach: A menu optimized for the Windows Notepad\texttrademark\ text editor}
\label{NotepadResult.PNG}
\end{figure}

\newpage

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{AcrobatUnoptimized.PNG}}
\caption{The Unoptimized menu for the Adobe Acrobat\texttrademark\ PDF viewer}
\label{AcrobatUnoptimized.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{AcrobatClassical.PNG}}
\caption{Dual-Objective MRF Approach: A menu optimized for the Adobe Acrobat\texttrademark\ PDF viewer}
\label{AcrobatClassical.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.5}
{\includegraphics{AcrobatResult.PNG}}
\caption{IFT-based Approach: A menu optimized for the Adobe Acrobat\texttrademark\ PDF viewer}
\label{AcrobatResult.PNG}
\end{figure}

\newpage

\begin{figure}[H] \centering
\scalebox{0.6}
{\includegraphics{FirefoxUnoptimized.PNG}}
\caption{The unoptimized menu for the Mozilla Firefox\texttrademark\ browser}
\label{FirefoxUnoptimized.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.6}
{\includegraphics{FireFoxClassical.PNG}}
\caption{Dual-Objective MRF Approach: A menu optimized for the Mozilla Firefox\texttrademark\ browser}
\label{FirefoxClassical.PNG}
\end{figure}

\begin{figure}[H] \centering
\scalebox{0.6}
{\includegraphics{FirefoxResult.PNG}}
\caption{IFT-based approach: A menu optimized for the Mozilla Firefox\texttrademark\ browser}
\label{FirefoxResult.PNG}
\end{figure}

\newpage

We note that the MRF-based menu for Notepad has fewer tabs than the baseline
(commercial) design.
This happens because the data instance of
Notepad involved high association scores between commands. 
Comparatively, the association values between pairs of
commands for Acrobat and Firefox were relatively lower. This sparse
association led to a wider layout with more tabs and smaller groups in
MRF-based menus. The same argument extends to the Acrobat menu: we see two
large-sized groups in the first and second tabs of Acrobat. The constituent commands of these groups
have highest association among each other. 
In addition, the association
scores of these commands are the only case where associations are relatively
high for that data instance. Thus, the dual-objective MRF is quite
strongly driven by the relative association values. 
But if we had set the $\lambda$ values in Subsection \ref{Classical Objective Function for MRF} differently, that formulation would not have valued the associations scores so much. We learn that the dual-objective formulation is quite sensitive to the $\lambda$ values.

Looking at the final results of MRF, it is difficult to justify the placement of
a specific command at the location suggested by the optimal solution.
Further analysis of the optimizer showed that we often had multiple different
feasible solutions within a narrow range of objective values.
However, the specific relative weightage of the two primary terms in the
objective function led to a situation where an odd/unexpected placement reported
in a slightly higher objective value. For example, the lead elements of most
groups in the Adobe Acrobat menu in MRF are quite esoteric and unrepresentative.
We conclude that the dual objectives of the MRF approach (weighted
performance by Fitts' law and mutual association of commands) led to a
relatively opaque and intractable objective function.
We also note that the dual-objective MRF did not address preferential
placement of commands in desirable tab location. 
The final placement does not fit common expectations. 
For example: the last/right-most tab
of the Firefox menu has the Cut-Copy-Paste commands and not the
Help-About commands commonly expected here.

Results from IFA appear to show a much
better balance between tab count and group size than the MRF for Notepad and
also for Adobe Acrobat. Even the Firefox, IFA menu is well balanced
except for the first tab (which gets skewed due to a large-sized group).
Overall, we appreciate and justify the positioning of commands and groups
based on the frequency of usage, association and also the standard
expectation of command positions.

Our analysis of the optimizer results for IFA shows that there exist relatively
fewer \textit{different} feasible solutions in near vicinity of the optimal solution.
This means that the formulation does not seem to be strongly affected by minor
variations in the relative weights of objective terms. This observation provides
a major advantage in cases where the weights cannot be deduced a-priori.

While satisfying the restrictions of computational performance, the
IFA based formulation provided well-organized results with good control on
loners and also on preferential placement of elements in tabs. In the next
section, we will explore whether these observations correlate with empirical user performance.

